Federated Neural Architecture Search

To preserve user privacy while enabling mobile intelligence, techniques have been proposed to train deep neural networks on decentralized data. However, training over decentralized data makes the design of neural architecture quite difficult as it already was. Such difficulty is further amplified when designing and deploying different neural architectures for heterogeneous mobile platforms. In this work, we propose an automatic neural architecture search into the decentralized training, as a new DNN training paradigm called Federated Neural Architecture Search, namely federated NAS. To deal with the primary challenge of limited on-client computational and communication resources, we present FedNAS, a highly optimized framework for efficient federated NAS. FedNAS fully exploits the key opportunity of insufficient model candidate re-training during the architecture search process, and incorporates three key optimizations: parallel candidates training on partial clients, early dropping candidates with inferior performance, and dynamic round numbers. Tested on large-scale datasets and typical CNN architectures, FedNAS achieves comparable model accuracy as state-of-the-art NAS algorithm that trains models with centralized data, and also reduces the client cost by up to two orders of magnitude compared to a straightforward design of federated NAS.

==> header.tex <==
% !TeX root = main.tex

%
%\usepackage{epsf,epsfig,textcomp,amsmath,amssymb,subfigure,cite,moreverb}

%\usepackage[table,xcdraw,dvipsnames]{xcolor} % xzl: if want to use auto gen table from  http://www.tablesgenerator.com

\usepackage{wrapfig}
\usepackage{comment}
%\usepackage{array}
\usepackage{colortbl}
\usepackage{cite}   % compact citations. does not work with showkeys

%\usepackage{hyperref}
\usepackage{tabularx}
\def\UrlBreaks{\do\/\do-}

% https://tex.stackexchange.com/questions/2369/why-do-the-less-than-symbol-and-the-greater-than-symbol-appear-wrong-as
% \usepackage[T1]{fontenc} % ensure > < to show up properly

%\usepackage[T1,hyphens]{url}
%\usepackage[colorlinks,urlcolor=blue]{hyperref}
%\usepackage{url}

%\usepackage{times}
\usepackage{color,soul}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{lipsum}

% http://latex-my.blogspot.com/2010/06/cjk-support-in-latex.html
\usepackage{CJKutf8} % JAP, CHN, KOR

\usepackage{tikz}
\usetikzlibrary{decorations.pathmorphing, patterns,shapes,snakes} % for zigzag, etc.

% \usepackage{enumitem}	% for fine control of list env
\usepackage[inline]{enumitem}	% for fine control of list env. support inline enumerate. 
\usepackage{listings} % for code listing
%
%\usepackage{booktabs}	% xzl: for fancy tables
\usepackage{lipsum}

\usepackage{capt-of}	% xzl: used to override the ``figure'' and ``table'' in caption.

%\usepackage{todonotes}  %xzl: for "missing figures"  NOTE this slows down compilation

\usepackage{ulem}  % xzl: for strikeout, which seems more robust than \st{} provided by soul package. 

% --- subcaption, can't be handled well if we output html -- 
%  xzl: for subfigure. incompatible with package subfig
\ifdefined\HCode
\usepackage[compatibility=false]{caption}
\def\pgfsysdriver{pgfsys-tex4ht.def}
\else
\usepackage{subcaption} 
\fi

% --- all sorts of math fonts ---
% cf: https://tex.stackexchange.com/questions/58098/what-are-all-the-font-styles-i-can-use-in-math-mode
\usepackage{mathrsfs}	% xzl: for Ralph Smith’s Formal Script Font (rsfs)
\usepackage{amsfonts}
%\usepackage{inconsolata} % xzl: this uses inconsolata for texttt -- conflict w ACM temp? already defined tt?

\usepackage[export]{adjustbox} % xzl: flush figure to left/right


% dvipsnames: more colors. however this option may clash with one defined in template
%\usepackage[dvipsnames]{xcolor} 


%
%%\usepackage[bookmarks, breaklinks=true, colorlinks=true, plainpages = false,
%%  citecolor = blue, urlcolor = blue, filecolor = blue,]{hyperref}
%
%\usepackage[labelfont=bf,font=medium]{caption}
%\usepackage[labelfont=bf,textfont=normalfont]{caption}
%\usepackage{multirow}
%
%\definecolor{tableYellow}{rgb}{.996, 1, .8549}
%\definecolor{tableBlue}{rgb}{0.8823, .9098, 1}
%\definecolor{tableRed}{rgb}{1, .9255, .9019}
%\definecolor{tableGreen}{rgb}{.9176, 1, .9216}
%\definecolor{tableGray}{rgb}{.902, .902, .902}
\definecolor{myForestGreen}{RGB}{34, 139, 34}
%
%\renewcommand\section{\@startsection {section}{1}{\z@}%
%   {-3ex \@plus -1ex \@minus -.2ex}%
%   {1.7ex \@plus.2ex}%
%   {\normalfont\large\bfseries}}
%\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%   {-2ex\@plus -1ex \@minus -.2ex}% used to be -2.5
%   {1ex \@plus .2ex}%
%   {\normalfont\normalsize\bfseries}}
%\renewcommand\subsubsection{\@startsection{subsubsection}{2}{\z@}%
%   {-1ex\@plus -1ex \@minus -.2ex}%
%   {0.3ex \@plus .2ex}%
%   {\normalfont\normalsize\bfseries}}
%
%\newcommand\minisection{\@startsection{subsubsection}{4}{\z@}%
%   {1ex\@plus 0ex \@minus 0ex}%
%   {-1.5ex \@plus .2ex}%
%   {\normalfont\normalsize\bfseries}}
%

% ----------- drawing --------------
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,fill=black,draw,text=white,inner sep=1pt] (char) {#1};}}
%\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%		\node[shape=circle,fill=airforceblue,draw,text=white,inner sep=1pt] (char) {#1};}}


% https://stuff.mit.edu/afs/athena/contrib/tex-contrib/beamer/pgf-1.01/doc/generic/pgf/version-for-tex4ht/en/pgfmanualse9.html
\newcommand*\snakezigzag		
{\tikz
%\draw[decoration = {zigzag,segment length = 0.35cm, amplitude = 0.9mm},decorate,very thin] (0,1.5) -- (1.5,1.5);
\draw[snake=zigzag,thick] (0,1.5) -- (1,1.5);
}

\newcommand*\snaketriangles
{\tikz
\draw[snake=triangles,thick] (0,1.5) -- (1,1.5);
}

\newcommand*\snakebump
{\tikz
\draw[snake=bumps,thick] (0,1.5) -- (1,1.5);
}

% \usepackage[color]{showkeys}	 % xzl: comment this out in final draft

%\definecolor{refkey}{RGB}{34,139,34}
%\definecolor{labelkey}{rgb}{0,0,1}

%\definecolor{refkey}{RGB}{34,139,34}
%\definecolor{labelkey}{rgb}{0,0,1}

		
%%------------Formatting----------
% nb: \paragraph{} is built-in and will affect many things --- 
\newcommand{\Paragraph}[1]{\vskip 3pt\noindent\textbf{#1 }}	 % used to be 6pt
%\newcommand\paratitle[1]{\textit{\textbf{#1}}}
\newcommand\paratitle[1]{\textit{\textbf{#1}} \hspace{1mm}}
%\newcommand{\Paragraph}[1]{\vskip 3pt\noindent\textbf{#1 }}	
%\newcommand\itno[1]{({\em #1})}
%\newcommand\itemno[1]{({\em #1})}

% @paragraph seems built-in. 
\renewcommand{\paragraph}[1]{\vskip 3pt\noindent\textbf{#1 }}	 % used to be 6pt


\renewcommand{\st}[1]{\sout{#1 }}	 % st{} from soul not robust enough

%%%%%%%%%%%%%%%% smitemize %%%%%%%%%%%%%%%%%%%%
%
\newenvironment{smitemize}%
  {\begin{list}{$\bullet$}%
     {\setlength{\parsep}{0pt}%
      \setlength{\topsep}{0pt}%
      \setlength{\itemsep}{2pt}}}%
  {\end{list}}
%
%%%%%%%%%%%%%%%% custom spacing %%%%%%%%%%%%%%%%%%%%
%
%----------- Comments-----------------
\newcommand\note[1]{\sethlcolor{yellow} \hl{#1}} % highlighted notes of other colors.
						 % For colors info from xcolor package, check out:
						 % http://en.wikibooks.org/wiki/LaTeX/Colors
\newcommand\Note[1]{\sethlcolor{green} \hl{#1}} % highlighted notes of other colors.						 
%\newcommand\note[1]{} % remove highlights.						 
\newcommand\notettx[1]{\sethlcolor{orange} \hl{#1}} % highlighted notes of other colors.

\newcommand\improve{\note{improve}}

\newcommand\xzl[1]{\sethlcolor{Dandelion} \hl{xzl: #1}} % highlighted notes of other colors.
\newcommand\todo[1]{\sethlcolor{myForestGreen} \hl{todo: #1}} % highlighted notes of other colors.

\newcommand\mj[1]{{\color{ForestGreen}{mj: #1}}}
\newcommand\mjD[1]{{\color{lightgray}{mj: #1}}}

\newcommand\hp[1]{{\color{blue}{hp: #1}}}
\newcommand\sz[1]{{\color{violet}{sz: #1}}}
\newcommand\lwg[1]{{\color{Emerald}
		{lwg: #1}}} % highlighted notes of other colors.
		
		
\newcommand{\textbfit}[1]{\textbf{\textit{#1}}}
		
%====== shortcut for ref ===== %
\newcommand\sect[1]{Section~\ref{sec:#1}}	% NB: does not play well with \note{}
		
%====== for estimating final pages ===== %
%\newcommand\ksm[1]{}
%\newcommand\ksmD[1]{}
%
%\newcommand\gena[1]{}
%\newcommand\genaD[1]{}
%
%\newcommand\xzl[1]{} % highlighted notes of other colors.
%
%\newcommand\mj[1]{}
%\newcommand\mjD[1]{}

% xzl: the one uses package enumitem that can fine tune indent.
% 
% for simplicity, can also use \begin{itemize}[leftmargin=*]
\newenvironment{myitemize}%
  {\begin{itemize}
	[leftmargin=0cm,
		itemindent=.3cm,
		labelwidth=\itemindent,
		labelsep=0pt,
		parsep=3pt,
		topsep=2pt,
		itemsep=1pt,
		align=left]
  }%
  {\end{itemize}}    

\newenvironment{myenumerate}%
  {\begin{enumerate}
	[leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,
		labelsep=0pt,
		parsep=1pt,
		topsep=1pt,
		itemsep=3pt,
		align=left]
  }%
  {\end{enumerate}}    
  
  % must turn on inline option for enumitem
\newenvironment{enumerateinline}%
  {\begin{enumerate*}
	[label=\roman*)]
  }%
  {\end{enumerate*}}      

\newenvironment{myenumerateinline}%
  {\begin{enumerate*}
	[label=\roman*)]
  }%
  {\end{enumerate*}}      
  
  
% -------------------FONTS-------------------
%\newcommand{\scenario}[1]{\textit{#1}}
\newcommand{\scenario}[1]{\texttt{#1}}

%\newcommand{\state}[1]{\texttt{#1}}

\newcommand{\system}[1]{\textsf{#1}}

% texttt will be larger than body text..
\newcommand{\code}[1]{\texttt{\small{#1}}}	
%\newcommand{\code}[1]{\texttt{#1}}	

\newcommand{\queue}[1]{\textit{#1}}
% ----------------------------------------------

%--------------------------------------------------------

\input{terms}

% Remove the copyright block space.
% http://ryanlei.wordpress.com/2012/02/13/latex-remove-the-copyright-space-from-the-acms-sig-alternate-template/
\makeatletter
\def\@copyrightspace{\relax}
\makeatother

